MILP initialization for solving parabolic PDEs with PINNs

Physics-Informed Neural Networks (PINNs) are a powerful deep learning method capable of providing solutions and parameter estimations of physical systems. Given the complexity of their neural network structure, the convergence speed is still limited compared to numerical methods, mainly when used in applications that model realistic systems. The network initialization follows a random distribution of the initial weights, as in the case of traditional neural networks, which could lead to severe model convergence bottlenecks. To overcome this problem, we follow current studies that deal with optimal initial weights in traditional neural networks. In this paper, we use a convex optimization model to improve the initialization of the weights in PINNs and accelerate convergence. We investigate two optimization models as a first training step, defined as pre-training, one involving only the boundaries and one including physics. The optimization is focused on the first layer of the neural network part of the PINN model, while the other weights are randomly initialized. We test the methods using a practical application of the heat diffusion equation to model the temperature distribution of power transformers. The PINN model with boundary pre-training is the fastest converging method at the current stage.

==> Nomenclature.tex <==
\section*{Nomenclature}

\begin{table}[]
    %\centering
    \begin{tabular}{lll}
$\lambda_u$ & & is the weight for the data loss function\\
$\lambda_f$ & &  is the weight for residual loss function\\

$n$ && is a reference number for input datapoint $n \in N$ \\
$N$ && is the size of an input dataset\\
$N_u$ && size of the input dataset for $MSE_u$\\
$N_f$ && size of the input dataset for $MSE_f$\\
$T$ && is the reference temperature \\
$\hat{T}$ && is the output temperature \\


    $f$ && \\
    
      
      MSE && Mean square error \\


      
      $n_{in}$   && number of input units  \\
      $n_{out}$ && number of output units \\

      $u$ && \\
    $W$ && weights \\
    $X^n$ && is the $n$-th input data point for MSE \\
    $\rho$ && is the density [kg/m$^3$] \\
    $c_p$ && is the specific heat capacity [J/kg$\cdot$K]\\
    $t$ && is the time reference point \\
    $x$ && is the spatial reference point \\
    $k$ && is the thermal conductivity [W/m$\cdot$K] \\
    $K$ && is the load factor [p.u.]\\
    $P_0$ && is the no-load loss [W]\\
    $P_K$ && is the load loss \\
    $h$ && is the convective heat transfer coefficient [W/m$^2 \cdot$K]\\
    %$\Delta_x$ && is a Laplacian \\
    $l$ && denote the layer number, $l \in L$\\ 
    $L$ && is the total number of layers \\
    $\sigma$ && is the neural network activation function \\
    $q$ && is \\
    $\hat{Y}$ && \\
    $b$ && denotes biases \\
    $MAE$ && is the Mean Absolute Error \\
    $j$ && is the \\
    $i$ && \\
    $\varepsilon$ && is \\
    
    \end{tabular}
   % \caption{Caption}
    \label{tab:my_label}
\end{table}
